Img2Vec: A Teacher of High Token-Diversity Helps Masked AutoEncoders

We present a pipeline of Image to Vector (Img2Vec) for masked image modeling (MIM) with deep features. To study which type of deep features is appropriate for MIM as a learning target, we propose a simple MIM framework with serials of well-trained self-supervised models to convert an Image to a feature Vector as the learning target of MIM, where the feature extractor is also known as a teacher model. Surprisingly, we empirically find that an MIM model benefits more from image features generated by some lighter models (e.g., ResNet-50, 26M) than from those by a cumbersome teacher like Transformer-based models (e.g., ViT-Large, 307M). To analyze this remarkable phenomenon, we devise a novel attribute, token diversity, to evaluate the characteristics of generated features from different models. Token diversity measures the feature dissimilarity among different tokens. Through extensive experiments and visualizations, we hypothesize that beyond the acknowledgment that a large model can improve MIM, a high token-diversity of a teacher model is also crucial. Based on the above discussion, Img2Vec adopts a teacher model with high token-diversity to generate image features. Img2Vec pre-trained on ImageNet unlabeled data with ViT-B yields 85.1\% top-1 accuracy on fine-tuning. Moreover, we scale up Img2Vec on larger models, ViT-L and ViT-H, and get $86.7\%$ and $87.5\%$ accuracy respectively. It also achieves state-of-the-art results on other downstream tasks, e.g., 51.8\% mAP on COCO and 50.7\% mIoU on ADE20K. Img2Vec is a simple yet effective framework tailored to deep feature MIM learning, accomplishing superb comprehensive performance on representative vision tasks.

==> chapter/chap3.tex <==
\section{Method} \label{sec:method}

\begin{figure*}
	\centering
	\subfloat{\includegraphics[width=0.96\linewidth]{images/show_fox.pdf}} \\
	\subfloat{\includegraphics[width=0.96\linewidth]{images/show_25.pdf}}
	\caption{\textbf{Visualization of targets similarity from different teachers.} The area with red box in first column is the \textit{query} patch. The right 6 columns are similarity heat-map of different teachers. Each grid indicates its similarity with the \textit{query}. The brighter the color, the greater the value, and vice versa. From left to right are MAE ViT-Base, MAE ViT-Large\cite{he2022masked}, SimCLR ResNet-50, SimCLR ResNet-101\cite{chen2020simple}, DINO ViT-Base and DINO ResNet-50\cite{caron2021emerging}.}
  \label{fig:teacher_token}
\end{figure*}

In this section, we start with a simple framework to reconstruct deep features in MIM task.
Based on the framework, we study how to choose a better teacher and introduce token diversity to estimate the features of teacher.
Then, we present our Img2vec framework with a high token diversity teacher and propose two novel modules, multi-block feature learning and global semantic learning, which improve the pre-training course. The Img2vec is illustrated in \cref{fig:Img2vec}.

\subsection{Deep Feature based MIM}

Recently, mask image modeling (MIM) is a impressive self-supervised visual learning method and draws great attentions in the research community. Some works (\eg MAE\cite{he2022masked}, MaskFeat\cite{wei2022masked}) use the pixel-level targets and reconstruct it from masked input. It's simple but lack of deep semantic information and yields weaker performance than deep feature based methods.
Using deep features as targets, BEiT\cite{bao2021beit} trains a feature code-book first and optimizes a classification task on the mask tokens. The code-book is quantized thus leads to loss details. data2vec\cite{baevski2022data2vec} and BootMAE\cite{dong2022bootstrapped} adopt a momentum updated model as teacher to extract target features. It's inflexible since the teacher must have the same structure with its student. And the hyper-parameter of momentum need be tuned carefully.

To address above problems, we introduce a simple MIM framework based on deep feature targets.
The whole framework is similar to MAE\cite{he2022masked} except the reconstruct target.
Mathematically, given an image $I$, it can be split into small patches $\left\{x_i\right\}_{i=1}^N$ and tokenized to hidden embeddings $\left\{h^0_i\right\}_{i=1}^N$. A random sampling mask on embeddings is generated and the masked tokens are dropped. Visible tokens are fed into a online encoder for pre-training. After the encoder, learnable mask tokens $m$ with position embeddings are added at corresponding mask position. A simple transformer is adopted as the decoder to reconstruct the targets. The targets is extracted from a teacher model with the intact image as its input. The teacher is a well-trained model and is not optimized during MIM learning.

Since the teacher can be replaced by any model, we will discuss how to choose a better teacher for MIM in \cref{sec:32}.

\subsection{Token Diversity for Teacher Evaluation} \label{sec:32}

% 放实验结果
\begin{table*}
  \centering
  \begin{tabular}{@{}ccccccc@{}}
  \toprule
  \multicolumn{2}{c}{Teacher} & Parameters & Linear probing & Fine-tuning & Diversity & Student top-1 Accuracy \\
  \midrule
  \multirow{2}{*}{MAE}    & ViT-Base/16   & 88M  & 68.0\% & 83.6\% & 0.530 & 84.3\% \\
                          & ViT-Large/16  & 307M & 75.8\% & 85.9\% & 0.587 & 84.4\% \\
  \midrule
  \multirow{2}{*}{SimCLR} & ResNet-50     & 26M  & 71.7\% & 76.3\% & 0.797 & 84.6\% \\
                          & ResNet-101    & 45M  & 73.6\% & 78.2\% & 0.752 & 84.2\% \\
  \midrule
                          & ViT-Base/16   & 88M  & 78.2\% & 82.8\% & 0.746 & 84.6\% \\
  \rowcolor{lightgray} \cellcolor{white}
  \multirow{-2}{*}{DINO}  & ResNet-50     & 26M  & 75.3\% & 77.4\%$^*$ & 0.831 & 85.0\% \\  
  \bottomrule
  \end{tabular}
  \caption{\textbf{Comparisons on teachers.} We present metrics on teacher models, including linear probe top-1  accuracy on ImageNet (Linear), fine-tuning accuracy (Finetune), token diversity (Diversity) and pre-trained ViT-B accuracy (Student Top-1). DINO ResNet-50 has the highest token diversity and the best student performance among all teachers. $^*$The fine-tuning accuracy is our reproducing result, which is not reported in the original paper.}
  \label{tab:teacher}
\end{table*}

When using our simple framework based on deep features, the teacher can be easily replaced with any trained model. Different teachers leads to various students' performance. Hence the question arises: \textit{How to evaluate the teacher for MIM task?} Intuitively, larger teacher models help the students learning better. However, using a ResNet\cite{he2016deep} may achieves better results than using a ViT as teacher.

To compare different teachers fairly, we conduct a series of experiments under the same pre-training and fine-tuning protocol. ViT-B\cite{dosovitskiy2020image} is adopted for comparison with $1600$ training epochs. We use random masking strategy with $60\%$ mask ratio and $32\times 32$ mask block size, and other settings are following MAE\cite{he2022masked}.

In order to compare teachers comprehensively, we consider $6$ pre-trained models from $3$ representative self-supervised approaches. Models using additional data or labeled data are excluded (\eg CLIP\cite{radford2021learning}, fine-tuned ResNet\cite{he2016deep}).
Teacher models for comparisons are:
\begin{itemize}
    \item \textbf{MAE\cite{he2022masked}}. The most representative pre-training method with mask image modeling. It optimizes the masked patch to reconstruct the image pixels. Model is trained on patch-level and lack of global learning. It achieves stronger results than all contrastive learning methods. MAE trained models on ViT\cite{dosovitskiy2020image}, and we use ViT-B/16 and ViT-L/16 as teachers.
    
    \item \textbf{SimCLR\cite{chen2020simple}}. A simple but effective framework of contrastive learning. It uses the same encoder to extract features from two augmented views of a image. All samples from the whole batch are collected to generate negative pairs for cross-entropy loss. SimCLR shows good results of contrastive learning methods. It provides pre-trained models on ResNet, and we use ResNet-50 and ResNet-101 for experiments.
    
    \item \textbf{DINO\cite{caron2021emerging}}. A powerful self-supervised method with self-distillation. It extracts the feature from the student model with heavy augmented image, and also obtains the features from the momentum updated model with multiple other views. A [CLS] token is adopted for aggregating embeddings from all other tokens. The cross-entropy loss on features of positive pairs is used for optimizing. Different from other contrastive learning method, DINO do not need negative pairs. It also achieves superb performance. We use ViT-B/16 and ResNet-50\cite{he2016deep} during teacher studies.
\end{itemize}

Thanks to the frozen model design, the teacher's structure can break free from the limitations of ViT. When taking ViT-B and ViT-L as teacher model, we apply the same image size and patch size for both student and teacher, which is $224^2$ and $16^2$ respectively. The targets dimension of ViT-B and ViT-L is $768$ and $1024$ correspondingly. The last layer outputs are directly adopted as the reconstruction targets.
When taking ResNet-50 and ResNet-101 as teacher, the model will output a $32\times$ down sampling rate feature map (\eg output $2048\times7\times7$ when input $3\times224\times224$). In order to keep the sequence length between student and teacher, we resize the input image from $224^2$ to $448^2$ with bilinear interpolation. Same as ViT, we take the features from last layer as targets.

The results are summarized in \cref{tab:teacher}, and the last column is top-1 fine-tuning accuracy of the student they taught. As for MAE, the ViT-L teaches a better student than ViT-B ($84.8\% vs. 84.3\%$), which is in line with the perception that larger model can distill better model in the knowledge distillation field. But surprisingly in DINO, The small ResNet-50 teacher gets a remarkable improvement compared to the big ViT-B teacher ($85.0\% vs. 84.6\%$), and even outperform the larger MAE ViT-L teacher ($85.0\% vs. 84.8\%$). This interesting phenomenon impels us to further study what property of the targets provided by teacher models leads to the different MIM performance.

The role of teacher is to provide reconstruction targets for student, thus we pay more attention on analysing these targets. We first visualize the relationship of target tokens by computing their pairwise cosine similarity, as shown in \cref{fig:teacher_token}. The area with red box in first column is the \textit{query} that calculate similarity with other tokens. The $2$--$7$ columns shows the response of $6$ different teacher models.

In \cref{fig:teacher_token}, we show a foreground \textit{query} and a background \textit{query} on two images. Compared to other models, the output tokens of DINO ResNet-50 reveal a stronger diversity. We hypothesize this property is important to MIM. MIM is the task that wants the model to reconstruct masked patches with visible patches, if the prediction targets are highly similar to each other, the model can easily use the visible patch's feature to predict the masked feature without regard to their semantics and contexts. For example, if the patch of fox's ear is masked, shown as first column in \cref{fig:teacher_token}, the MAE based teacher could tolerate student predicting it as fox's body feature, while the DINO based teacher requires the student predicting more accurate. The token diversity suggests a discriminative ability for understanding different visual areas.

Also, we present a quantitative analysis of token diversity. For a teacher feature sample with $N$ tokens $\{y_i\}_{i=1}^N$, we compute the pairwise cosine similarity between all tokens and use min-max normalization to map the value into $[0,1]$. Then we average these similarities for the sample. Finally, we scan the whole ImageNet-1K train set with $N$ samples and get the diversity $diver = 1 - \frac{1}{N} \sum_{i=1}^N {sim}_i$, where ${sim}_i$ is the similarity for sample $i$. A larger $diver$ value means tokens distribute more diverse.

\cref{tab:teacher} shows the quantitative properties of teachers. 
Our results suggest that the token diversity is an effective metric to measure the targets quality in MIM task, and it sometimes even plays a more important role than other properties, such as model performance and capacity.
Under the same network structure, the teacher with higher token diversity teaches a better student (\eg DINO ViT-B \textit{vs} MAE ViT-B, DINO ResNet-50 \textit{vs} SimCLR ResNet-50). It is worth noting that the smaller teacher, DINO ResNet-50, can provide more appropriate reconstruction targets than MAE ViT-L, which has a larger model capacity and a stronger feature extraction capability.

Furthermore, we present t-SNE\cite{van2008visualizing} visualization for MAE ViT-B and DINO ResNet-50 teachers. Since both teachers have different feature dimensions, we first adopt PCA\cite{pearson1901liii} to reduce the dimensions to $128$, and then use t-SNE to embed them into the same manifold. The visualization result is shown in \cref{fig:t-sne}, and the DINO ResNet-50 tokens is more dispersed which get a higher token diversity.

\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth]{images/t-sne.pdf}
  \caption{\textbf{t-SNE visualization.} We take the tokens of the fox image and show their distribution of MAE ViT-Base and DINO ResNet-50. The tokens extracted by DINO ResNet-50 reveal a stronger diversity.}
  \label{fig:t-sne}
\end{figure}

\subsection{Img2vec}

According to above target selection discussion, we adopt the high token diversity model, DINO ResNet-50, as our target model. Further, we propose our Img2vec framework for MIM task. It is based on aforementioned simple framework and contains two novel modules, multi-block feature learning and global semantic learning. The overall framework is presented in \cref{fig:Img2vec}.

\textbf{Multi-block feature learning.} In pre-training, a encoder-decoder structure is adopted. Typical encoder only passes its last block feature to the decoder and the early blocks not optimized well from the decoder. To train more effective, we propose multi-block feature learning. The embeddings of all encoder blocks are averaged into the encoder output,
$h_{i} = \sum_{l=1}^L h_{i}^{l}$,
where $i$ denotes the patch index and $l$ is the layer index. And the early features can be fed into the decoder directly. 

To reconstruct the targets, a simple 2-layers transformer with one linear projection layer is adopted as a decoder. It takes the multi-block feature as input, and outputs the predictions with the patch loss. The patch loss is smooth l1 loss\cite{girshick2015fast} and calculates on all masked patches,
\begin{equation}
    L_{\text{patch}} = \frac{1}{\Omega(\mathcal{M})} \sum_{i \in \mathcal{M}} \text{smooth}_{L_1} (y_i - z_i)
\end{equation}
where $y$ is the targets extract by the target model, $z$ is the predictions of decoder, $\mathcal{M}$ is the indices of masked patches, and $\Omega(\cdot)$ means the cardinals of set.

\textbf{Global semantic learning.} MIM is the task that makes model learning through predicting the masked areas under a patch-level supervision. This strategy may divert the model from understanding the visual sense in a whole image perspective, thus limits the performance. We introduce the global semantic learning to our Img2vec through an additional global loss. We calculate the smooth $L_1$ loss between the global embeddings of target and pre-trained model. 
The target model's global embedding is the mean of $N$ tokens $\{y_i\}_{i=1}^N$. 
For the pre-trained model, we first use a simple MLP, including 2 linear layer with one ReLU\cite{nair2010rectified} layer, as a projector head $p$ to project $M$ visible tokens $\{h_i\}_{i=1}^M$ of the encoder's last layer to the target's dimension space. Then the encoder global embedding is obtained by averaging these tokens, and thus the global loss is:
\begin{equation}
L_\text{global} = \text{smooth}_{L_1}(\frac{1}{\Omega(\mathcal{M})} \sum_{i \in \mathcal{M}}p(h_i) - \frac{1}{N}\sum_{i=1}^{N}y_i).
\end{equation}
We note that the [CLS] token does not participate in the computation for global embeddings.
The design of global semantic is simple and intuitive, we get the global embedding in a similar manner as ViT do in the classification task, which take a average pooling to the backbone's output as image-level representation for the subsequent classifier.

Global semantic implicit adopts two masked views of one image as positive pair, because of their same optimal objective. It desires a small distance between positive pairs, and thus improves the feature from the same instance clustering closer.

Overall, the total loss of our Img2vec is:
\begin{equation}
    L = L_\text{patch} + \lambda L_\text{global}.
\end{equation}
The $\lambda$ is a hyper-parameter to balance the global semantics.

